Scene Coordinate and Correspondence Learning for Image-Based Localization

Scene coordinate regression has become an essential part of current camera re-localization methods. Different versions, such as regression forests and deep learning methods, have been successfully applied to estimate the corresponding camera pose given a single input image. In this work, we propose to regress the scene coordinates pixel-wise for a given RGB image by using deep learning. Compared to the recent methods, which usually employ RANSAC to obtain a robust pose estimate from the established point correspondences, we propose to regress confidences of these correspondences, which allows us to immediately discard erroneous predictions and improve the initial pose estimates. Finally, the resulting confidences can be used to score initial pose hypothesis and aid in pose refinement, offering a generalized solution to solve this task.

==> contents/evaluation.tex <==
\section{Experimental Setup}
In this section, we first describe how the dataset is generated by combining simulated object renderings with background noise and real images taken from the LineMOD dataset \cite{hinterstoisser2012model}. Then we give an overview of our experimental setup before demonstrating and evaluating the results.
\subsection{Dataset Generation}
Since both former closely related feature descriptor learning and pose estimation methods used the LineMOD dataset for their experiments, we also chose this dataset to be able to evaluate the algorithm's performance. 

The LineMOD dataset consists of fifteen distinct 3D mesh models and respective RGB-D sequences of them together with the camera poses. These data are used to create training set $S_{train}$, database set $S_{db}$, and test set $S_{test}$ each consisting of samples $\textbf{s} = (\textbf{x}, c, \textbf{q})$, where $\textbf{x}$ stands for the depth image patch, $c$ and $\textbf{q}$ are the corresponding class and pose, respectively. The training set $S_{train}$ as its name suggests used exclusively for training. The database set $S_{db}$ is used for the evaluation phase, where its samples are used to construct a descriptor database used for the nearest neighbor search, whereas $S_{test}$ is used exclusively in the evaluation phase.


First, we render each of the fifteen objects from different viewpoints covering their upper hemisphere, depicted in Fig. \ref{fig:normal}. Here, following previous methods \cite{wohlhart2015learning,zakharov2017}, viewpoints are defined as vertices of an icosahedron centered around the object. By repeatedly subdividing each triangular face of the icosahedron additional viewpoints and, therefore, a denser representation can be created. In our case, the training set $S_{train}$ sampling is achieved by recursively applying three consecutive subdivisions on the initial icosahedron structure (see Fig. \ref{fig:normal}). Furthermore, following the method of \cite{zakharov2017}, we add in-plane rotations at each vertex position by rotating the camera at each sampling vertex from -45 to 45 degrees using a stride of 15 degrees.

As a next step, we extract patches covering the objects from both rendered images and real images coming from the depth sequences. The bounding box is defined by the bounding cube size of 40 \si{cm^{3}} centered on the object. All the values beyond the bounding cube are clipped. Upon extraction of the patches, each of them is being normalized, mapped to the range of $[0, 1]$ and stored together with its identity class $c$ and pose $\textbf{q}$ resulting in a single sample $\textbf{s}$.

The training set $S_{train}$ is then generated by combining all the samples coming from the rendering and $50\%$ of the real data from the depth sequences (resulting in approximately $18\%$ of the real data in $S_{train}$). The selection of the real samples is performed by choosing the most similar poses to the ones used for synthetically rendered samples. The rest of the real samples are used to generate the test set $S_{test}$. The database set $S_{db}$ contains only the synthetic part of the $S_{train}$.

\begin{figure}[!htbp]
	\centering
	\begin{subfigure}[b]{.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{images/cat}
		\caption{Regular}
		\label{fig:normal}
	\end{subfigure} \hfill
	\begin{subfigure}[b]{.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{images/eggbox}
		\caption{Symmetric}
		\label{fig:symmetric}
	\end{subfigure} \hfill
	\begin{subfigure}[b]{.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{images/bowl}
		\caption{Rotation-inv.}
		\label{fig:rotinv}
	\end{subfigure}
	\caption{Sampling points for different objects types: vertices represent camera positions from which the object is rendered.}
	\label{fig:samplings}
\end{figure}

\subsubsection{Treating Rotation-invariant Objects}
Four out of fifteen objects of the LineMOD dataset have a property of rotation-invariance and introduce an ambiguity to the generation of triplets needed for the triplet classification loss. For instance, the \textit{bowl} object is fully rotation-invariant, whereas the \textit{cup}, \textit{eggbox} and \textit{glue} object are only rotation-invariant around a single plane or, in other words, symmetric. These four objects need to be treated differently from the rest. This comes from the fact that, in the case of rotation-invariant objects, samples representing different poses might look exactly the same, which can result in a faulty triplet required for the triplet loss function. 

To solve this problem, we render only a limited amount of poses for those objects, such that every image patch is unique. Sample vertices for different object types are demonstrated in Fig. \ref{fig:symmetric} and \ref{fig:rotinv}. Since both training set $S_{train}$, and test set $S_{test}$ also include real samples we also omit ambiguous poses in them and only consider those that are close to the ones coming from the renderer. Note that this sampling also results in an unbalanced percentage of real images included for each object. To consider this, we create datasets of five, ten and fifteen objects and only include the rotation-invariant objects when using the full LineMOD dataset of fifteen objects.

\subsubsection{Data Augmentation}
The synthetic samples coming from the renderer have a black background, which makes them very different from the real samples. Since we have a limited amount of the real data available and cannot cover all the possible poses, we augment the training samples with a background noise whenever the real sample for this pose is not available. Augmented samples are included in the training set $S_{train}$ during training in an online fashion, generating different noise patterns for each anchor sample. The noise type we use for our pipeline is purely synthetic and is present in both \cite{wohlhart2015learning} and \cite{zakharov2017} showing the best performance among synthetic noise types. It is referred to as fractal noise and is based on a combination of several octaves of simplex noise first introduced in \cite{perlin2001noise}. It provides a smooth non-interrupting noise pattern and is often used for landscape generation by game developers. 

%\begin{figure}[h]
%	\begin{center}
%		\includegraphics[width=0.8\linewidth]{images/set.png}
%		\caption{Example triplets for the cat object of the LineMOD dataset and different %background types.}
%		\label{fig:set}
%	\end{center}
%\end{figure}

\subsection{Implementation Details}
With this training and testing setup, we extract patches of size $n=64$. We then train our CNN, where, if not stated otherwise, we use the network architecture introduced in \cite{wohlhart2015learning}, except we set the feature descriptor size to $d=64$. As it is mentioned in \cite{wohlhart2015learning} at some point increasing the feature descriptor size does not improve the methods performance anymore. As for regression we found a similar effect during our experiments, in which we experienced $d=64$ to be a good trade-off between nearest neighbor and regression performance. 
During our experiments, we set $\gamma=10.0$ for the dynamic margin. 
The network was trained on a Linux-based system with 64GB RAM and 8GB NVIDIA GeForce GTX 1080 graphics card. All experiments are implemented using TensorFlow\footnote{https://www.tensorflow.org/} with Adam optimizer and an initial learning rate of $1e^{-3}$, while the batch size was set to $300$.

\subsection{Baseline Models}
To analyze not only our method, but the effect of multi-task learning, i.e. regression and learning robust feature descriptors together, we report the results compared to the baseline method \cite{zakharov2017}. Here we train on the loss function $L_d$ to compare to the results obtained by nearest neighbor pose retrieval, abbreviated as \textit{NN}. However, in comparison, the baseline in their original work uses RGB-D data and includes normals as additional information whereas we only use depth information. Including surface normals as an additional input could give extra information, but as we optimize for depth images only in this paper, this should be further investigated in future work. Nevertheless, the authors provided us with an implementation of their pipeline written in python so that we were able to run all our experiments and compare the results using depth images only. 
In addition, we conduct our own baseline for regression only ($R$) and report the results. Furthermore, to evaluate our method, we report the results obtained by the end-to-end regression (\textit{Rours}), as well as the results obtained by using the resulting features for nearest neighbor lookup (\textit{NNours}). 
%Since we use depth images and include in-plane rotations, adding an additional degree of freedom, comparisons to \cite{wohlhart2015learning} as is, were not conducted.

\subsection{Evaluation Metrics}
To evaluate the performance of our method, we use the angular error comparing the ground truth pose $\textbf{q}$ and the predicted one $\hat{\textbf{q}}$ for a given test image $\textbf{x}_i$:

\begin{equation}
\theta(\textbf{q}_i, \hat{\textbf{q}_i}) = 2 \cdot arccos(|\textbf{q}_i \cdot \hat{\textbf{q}_i}|).
\end{equation}
The pose can either be obtained by nearest neighbor lookup or directly estimated by the neural network.
%In addition we report the geodesic distance:
%\begin{equation}
%    d_{geo}(q_i, \hat{q_i}) = \|log(R_i \hat{R_i^T})\|,
%\end{equation}
%where $R_i$ and $\hat{R_i}$ are the rotation matrices corresponding to quaternion $q_i$ %and $\hat{q_i}$. The geodesic distance results in values in $[0, \pi)$. %\cite{huynh2009metrics}\\
Furthermore, we report the angular accuracy, where each test image is considered a true positive if its angular error is below a threshold $t$, where $t \in [10, 20, 40]$ degrees.

Also, to evaluate the resulting feature descriptor we visualize the features in a lower dimensional space using PCA and t-SNE \cite{maaten2008visualizing}.

\section{Evaluation}
In this section, we first give a detailed analysis of our method compared to the baseline and discuss several aspects of our method, starting with the influence of the network architecture on the methods performance.
\subsection{Comparison to baseline method}
We first evaluated our method on models trained on a different number of objects, for which the mean angular error is reported in Table \ref{tab:results}. Note that for nearest neighbor pose retrieval only the poses of correctly classified objects are considered, while for regression the whole test set is used, as in this case we do not directly infer the class. 
%Compared to the nearest neighbor pose retrieval based on the feature descriptors obtained while training only on the $L_d$ loss, we report the angular error using regression only, meaning the model was only trained based on the $L_{pose}$ loss function. 
%For objects with little shape variation regressing the pose directly usually becomes a much more difficult task. However, by including our multi-task learning approach we were able to significantly improve the regression accuracy.

Overall, we experienced a significant improvement in performance for both regression as well as nearest neighbor search accuracy by our proposed method. During training, the usually more difficult regression task, seems to be optimized by additionally focusing on learning a meaningful embedding, improving the mean angular error by $28.8\%$. Since poses as well as objects are already well-distinguished and the feature descriptors separated by the triplets and pair loss functions, regression can more easily be learned. 

As for the performance of nearest neighbor search we found an improvement in robustness and accuracy of our multi-task learning framework compared to the baseline. The standard deviation as well as the mean angular error of our model, \textit{NNours}, decreases significantly, making the method more robust. Here we can report a relative improvement of $30.0\%$ for the mean angular error while training on the full LineMOD dataset, meaning fifteen objects.

Both regression and nearest neighbor method benefit from jointly learning robust features and poses. Which model to choose now becomes a trade-off between time complexity and accuracy, which we will address further in section \ref{sec:scalability}.
%We can observe an improvement in the resulting pose retrieval accuracy using the features obtained by manifold learning. In case the direct pose regression fails, we can still easily get a good pose estimate by using the nearest neighbor search. 
%\begin{figure*}[t]
%	\begin{center}
%		\includegraphics[width=0.8\linewidth]{images/comp_new}
%		\caption{Mean angular error for different objects comparing nearest neighbor pose retrieval \cite{zakharov2017}, regression and our proposed approach. Note that for fifteen as well as ten objects our proposed method improves the regression accuracy as well as the pose retrieval using nearest neighbor search on the descriptor space.}
%		\label{fig:benchvise}
%	\end{center}
%\end{figure*}

%\begin{table*}[t]
%    \begin{center}
%        %\vspace{0.4cm}
%        \begin{tabular}{|c|c|c|c|c|c|c|}
%            \hline
%            Method & 15 objects & classification & 10 objects & class & 5 objects  & class\\
%            \hline\hline
%            NN &  25.29(11.76)+-40.75&  92.46 & 19.98(10.58)+-34.78 & 92.56 & 24.19(10.72)+-43.34& 99.31\\
%            NNours & 17.70(11.59)+-25.78 & 97.07 & 14.74(11.53)+-15.04 & 97.50&13.05(10.29)+-15.19 & 99.90\\
%            R & 38.23(26.16)+-34.65 & -  & 29.17(20.69)+-28.03 & -&22.07(15.56)+-24.40 & -\\
%            Rours & 27.28(19-25)+-27.26 & -& 23.08(17.56)+-21.25 & - & 19.16(13.80)+-21.54 & -\\                   
%            \hline
%        \end{tabular}
%        \caption{Comparison between the angular error (Mean (Median) +- Std) of the baseline method \textit{NN}, regression and our approach.}
%        \label{tab:results}
%    \end{center}
%
%\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[h]
	\centering
	\resizebox{\textwidth}{!}{%
		%	\def\arraystretch{0.9}% 
		\begin{tabular}{@{}lcccccc@{}}
			\toprule
			& \multicolumn{2}{c}{\textbf{15 Objects}}                 & \multicolumn{2}{c}{\textbf{10 Objects}}                 & \multicolumn{2}{c}{\textbf{5 Objects}}                  \\ \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
			& \textbf{Mean (Median) $\pm$ Std} & \textbf{Classification} & \textbf{Mean (Median) $\pm$ Std} & \textbf{Classification} & \textbf{Mean (Median) $\pm$ Std} & \textbf{Classification} \\ \midrule
			\textbf{\textit{NN} \cite{zakharov2017}}     & 25.29$^{\circ}$ (11.76$^{\circ}$) $\pm$ 40.75$^{\circ}$           & 92.46\%                   & 19.98$^{\circ}$ (\textbf{10.58}$^{\circ}$) $\pm$ 34.78$^{\circ}$           & 92.56\%                   & 24.19$^{\circ}$ (10.72$^{\circ}$) $\pm$ 43.34$^{\circ}$           & 99.31\%                   \\
			\textbf{\textit{NNours}} & \textbf{17.70$^{\circ}$ (11.59$^{\circ}$) $\pm$ 25.78$^{\circ}$}           & \textbf{97.07\%}                   & \textbf{14.74$^{\circ}$} (11.53$^{\circ}$) $\pm$ \textbf{15.04$^{\circ}$}           & \textbf{97.50\%}                   & \textbf{13.05$^{\circ}$ (10.29$^{\circ}$) $\pm$ 15.19$^{\circ}$}           & \textbf{99.90\%}                   \\ \midrule
			\textbf{\textit{R}}      & 38.23$^{\circ}$ (26.16$^{\circ}$) $\pm$ 34.65$^{\circ}$           & -                       & 29.17$^{\circ}$ (20.69$^{\circ}$) $\pm$ 28.03$^{\circ}$           & -                       & 22.07$^{\circ}$ (15.56$^{\circ}$) $\pm$ 24.40$^{\circ}$           & -                       \\
			\textbf{\textit{Rours}}  & \textbf{27.28$^{\circ}$ (19.25$^{\circ}$)} $\pm$ \textbf{27.26$^{\circ}$}           & -                       & \textbf{23.08$^{\circ}$ (17.56$^{\circ}$)} $\pm$ \textbf{21.25$^{\circ}$}           & -                       & \textbf{19.16$^{\circ}$ (13.80$^{\circ}$)} $\pm$ \textbf{21.54$^{\circ}$}           & -\\              
			\bottomrule
		\end{tabular}
	}
	\caption{Angular error of the baseline method (\textit{NN}), regression (\textit{R}) and our approach (\textit{Rours, NNours}).}
	\label{tab:results}
	\vspace{-5pt}
\end{table*}

%\begin{table}[h]
%    \begin{center}
%        \begin{tabular}{|c|c|c|c|c|}
%            \hline
%            Accuracy & $10^{\circ}$ & $20 ^{\circ}$ & $40 ^{\circ}$  & class \\
%            \hline\hline
%            \textit{NN} & 34.92\% &  67.48\% & 79.11\% & 90.56\% \\
%            \textit{Ours} & 40.96\% &  82.68\% & 93.19\% & 96.41\% \\
%            \textit{Ours$_{deep}$} & 47.94 \% & 89.10 \% & 97.85 \% & 98.94 \%\\
%            \hline
%        \end{tabular}
%        \vspace{0.4cm}
%        \caption{Comparison between the accuracy of the baseline loss functions \cite{zakharov2017} \textit{NN} and our results on 10 objects of the LineMod dataset.}
%        \label{tab:ten_percent}
%    \end{center}
%    
%\end{table}
%For another experiment, we include ten objects in one model, excluding the rotation-invariant objects of the LineMOD dataset, as they introduce imbalance to the number of poses per object. We obtained similar results as can be seen in Table \ref{tab:ten_percent}. 

%\begin{table}[h]
%	\centering
	%        \setlength{\leftskip}{20pt}
	
%	\resizebox{1\linewidth}{!}{%
%		\def\arraystretch{1}%
%		\begin{tabular}{@{}lcccc@{}}
%			\toprule
%			\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{\textbf{Angular error}} & \multirow{2}{*}{\textbf{Classification}} \\ \cmidrule(lr){2-4}
%			\multicolumn{1}{c}{} &                 \textbf{10$^{\circ}$} & \textbf{20$^{\circ}$} & \textbf{40$^{\circ}$} &   \\
%			\midrule
			%\cmidrule(r){1-1} \cmidrule(l){5-5} 
%			\textbf{\textit{NN}} \cite{zakharov2017} & 42.39\% &  79.02\% & 86.52\% & 92.56\% \\
%			\textbf{\textit{NN\_ours}} & 38.74\% &  81.28\% & 95.03\% & 97.50\% \\
%			\textbf{\textit{NN\_ours$_{deeper}$}} & 47.94\% & 89.10\% & 97.85\% & 98.94\%\\ \bottomrule
%		\end{tabular}
%	}
%	\vspace{0.4cm}
%	\caption{Comparison between the classification and angular accuracy of the baseline method, \textit{NN}, and our results on 10 objects of the LineMod dataset.}
%	\label{tab:ten_percent}
%\end{table}
%\pagebreak

%It is worth noting, that using our end-to-end regression we are still able to obtain similar results as the baseline method that uses nearest neighbor pose retrieval. Meaning we are able to remove the need for storing a database, for which the memory consumption increases linearly with each additional object. With additional fine-tuning of our method, for example by optimizing the network architecture, we believe we can even further improve the regression accuracy. However, since the main purpose of this work is to analyze the effect of both manifold learning and regression in a multi-task framework, we conduct a small experiment but leave the main evaluation of this to future work.

Next, to analyze our resulting feature descriptors, we compare our method using nearest neighbor search, \textit{NNours} to the baseline method, for which we report the classification and pose accuracy in Table \ref{tab:percent}. Again, our experiment results show that the feature descriptors provided by the model trained on both tasks seem to be more distinguishable as well. As a result the nearest neighbor pose retrieval accuracy improves even further. Additionally, we are able to improve the classification accuracy compared to the state-of-the art methods.


%\begin{table}[h]
%    \begin{center}
%        \begin{tabular}{|c|c|c|c|c|}
%            \hline
%            Accuracy & $10^{\circ}$ & $20 ^{\circ}$ & $40 ^{\circ}$  & class \\
%            \hline\hline
%            \textit{NN} & 39.92\% &  75.39\% & 85.10\% & 94.94\% \\
%            \textit{Ours} & 34.73\% &  75.94\% & 89.23\% & 94.89\% \\
%            \textit{Ours$_{deep}$} & 39.81 \% & 78.57 \% &  90.87 \% & 95.70 \%\\
%            \hline
%        \end{tabular}
%        \vspace{0.4cm}
%        \caption{Comparison between the accuracy of the baseline loss function \cite{zakharov2017} \textit{NN} and our results on 15 objects of the LineMod dataset.}
%    \label{tab:percent}    
%    \end{center}
%    
%\end{table}

\begin{table}[h]
	\centering
	%        \setlength{\leftskip}{20pt}
	\resizebox{1\linewidth}{!}{%
		\def\arraystretch{1}%
		\begin{tabular}{@{}lcccc@{}}
			\toprule
			\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{\textbf{Angular error}} & \multirow{2}{*}{\textbf{Classification}} \\ \cmidrule(lr){2-4}
			\multicolumn{1}{c}{} &                 \textbf{10$^{\circ}$} & \textbf{20$^{\circ}$} & \textbf{40$^{\circ}$} &   \\
			\midrule
			%\cmidrule(r){1-1} \cmidrule(l){5-5} 
			\textbf{\textit{NN}} \cite{zakharov2017} & 35.98\% &  71.56\% & 82.72\% & 92.46\% \\
			\textbf{\textit{NNours}} & 37.89\% &  79.61\% & 92.27\% & 97.07\% \\
			\textbf{\textit{NNours$_{deeper}$}} & \textbf{41.32\%} & \textbf{82.52\%} &  \textbf{93.51\%} & \textbf{97.26\%}\\ \bottomrule
		\end{tabular}
	}
	\vspace{0.4cm}
	\caption{Comparison between the classification and angular accuracy of the baseline method, \textit{NN}, and our results on 15 objects of the LineMod dataset.}
	\label{tab:percent}    
\end{table}

\subsection{Influence of Network Architecture}
Additionally, to explore the methods performance using network architectures with varying depths, we run our model using the network architecture described in \cite{bui2017x}. This architecture is two layers deeper and removes max pooling layers by including convolutional layers with stride two. Stated by the authors of \cite{wohlhart2015learning}, a deeper network architecture did not seem to improve the accuracy of the method further, which we experienced in our test as well, however by using our multi-task learning framework and testing on a deeper network architecture we found that we can improve the pose estimation accuracy even further. Here we were able to achieve the results seen in Table \ref{tab:percent}, abbreviated as {\textit{NNours$_{deeper}$}. We report a relative improvement of $7.2\%$ using nearest neighbor search and $9.0\%$ in the mean angular error of our regression results by using a deeper network architecture, while training on the full LineMOD dataset. However, further experiments should be conducted to analyze and optimize the network and assess the effect on the regression accuracy.
	
	%\begin{figure}[h]
	%	\begin{center}
	%		\includegraphics[width=0.99\linewidth]{images/angle_error_new}
	%		\caption{Mean angular error of nearest neighbor pose retrieval, regression and our approach, evaluated during training on the test set.}
	%		\label{fig:angle_error}
	%	\end{center}
	%\end{figure}
	
	%The same trend can be seen during training when evaluating the current model on the test set. %Both regression and nearest neighbor pose retrieval accuracies benefit from multi-task %learning, which is depicted in Fig. \ref{fig:angle_error}. One can see nicely that using our %approach the accuracy for both regression as well as the pose found using nearest neighbor %search on the resulting feature descriptors is improved by a significant amount. Furthermore, %by including only a few additional layers to the network it can be seen that for both %regression and nearest neighbor search the performance increases even further and that we can %get similar results using regression as compared to the nearest neighbor search baseline.
	%\%begin{table}[h]
	%    \begin{center}
	%        \begin{tabular}{|c|c|c|c|c|}
	%            \hline
	%            Accuracy & $10^{\circ}$ & $20 ^{\circ}$ & $40 ^{\circ}$ & classification \\
	%            \hline\hline
	%            10 objects & 47.94 \% & 89.10 \% & 97.85 \% & 98.94 \%\\
	%            15 objects & 39.81 \% & 78.57 \% &  90.87 \% & 95.70 \%\\
	%            \hline
	%        \end{tabular}
	%        \vspace{0.4cm}
	%        \caption{Results on 10 and 15 objects of the LineMOD dataset using a deeper network architecture.}
	%        \vspace{0.4cm}
	%    \label{tab:deepercnn}
	%    \end{center}
	
	%\end{table}
	\subsection{Feature Visualization}
	As we have shown in our experiments, apart from the improvement in accuracy for pose regression, we experienced an increase in the performance of nearest neighbor pose retrieval as well. To analyze the resulting feature descriptors, we visualize the descriptors in the lower dimensional 3D-space using PCA and t-SNE. 
	
	%\begin{figure}[h]
	%    \begin{center}
	%        \includegraphics[width=0.49\linewidth]{images/pca.png}
	%        \includegraphics[width=0.49\linewidth]{images/t-sne.png}
	%        \caption{Feature visualization using left: PCA and right: t-sne.}
	%        \label{fig:fvis}
	%    \end{center}
	%\end{figure}
	
	We use TensorBoard\footnote{https://www.tensorflow.org/get\_started/embedding\_viz} to create the visualizations. For t-SNE, we use a perplexity of $100$, learning rate of $10$ until convergence. Using PCA, the variance including the best three components resulted in $53.2\%$. The resulting clusters for five objects can be seen in Fig. \ref{fig:fvisreg}, as well as in the videos included in the supplementary material. We observe that in both cases the object classes are nicely distinguished using feature descriptors obtained by our proposed approach. 
	
	\subsection{Scalability}
	\label{sec:scalability}
	In this section we analyze the time complexity and accuracy of our models at different number of objects. For nearest neighbor search we use a standard OpenCV matcher. Fig. \ref{fig:scalability} shows the mean time of our models and the corresponding angular error. The mean time for regression is calculated as one forward pass of the neural network. For nearest neighbor methods only the matching time is tracked. To obtain the total time needed, the time of one forward pass should be added to the shown results for matching. One can see nicely that regression has a constant time, regardless of how many objects are used, whereas for nearest neighbor searches the time increases with additional objects. Depending on the application, this and the drop in accuracy for additional objects should be taken into account.
		\begin{figure}[b]
			\begin{center}
				\includegraphics[width=0.97\linewidth]{images/scalability}
				\caption{Average time and median angular error of nearest neighbor pose retrieval, regression and our approach evaluated on ten objects of the LineMOD dataset.}
				\label{fig:scalability}
			\end{center}
		\end{figure}
	
%	\subsection{Adaption to Detector}
%	%\begin{table*}[t]
%	%    \begin{center}
%	%        \caption{Comparison between results obtained by using different bounding box sizes.  The \textbf{median} angular error for tight, 0.2 and 0.3 diameter size is reported.}
%	%        \vspace{0.4cm}
%	%        \begin{tabular*}{0.915\textwidth}{|c|c|c|c|c|c|}
%	%            \hline
%	%            Method & Benchvise & Driller & Cat & Iron & 10 objects\\
%	%            & tight - 0.2 - 0.3 &  tight - 0.2 - 0.3 &  tight - 0.2 - 0.3 &  tight - 0.2 - 0.3&  tight - 0.2 - 0.3\\
%	%            \hline\hline
%	%            $NN_m$ & 9.46 - $^{\circ}$&  $^{\circ}$&  9.30 - 9.91 $^{\circ}$&  8.81 - $^{\circ}$&  12.00 - 10.58$^{\circ}$\\
%	%            $NN_{ours}$ & 9.64 - $^{\circ}$&  $^{\circ}$&  10.47 - 9.93 $^{\circ}$&  8.95 - $^{\circ}$& 11.01 - 11.53 $^{\circ}$\\
%	%            $R{ours}$ &  9.40 - $^{\circ}$& $^{\circ}$& 9.65 - 8.78 $^{\circ}$& 8.72 - $^{\circ}$&  20.25 - 17.56$^{\circ}$\\
%	%            \hline
%	%        \end{tabular*}
%	%        \label{tab:bb}
%	%    \end{center}
%	%\end{table*}
%	\begin{figure*}[t]
%		\begin{center}
%			\includegraphics[width=0.8\linewidth]{images/bb_new}
%			\caption{Comparison between results obtained by using different bounding box sizes. The mean angular error for tight, tight but distorted, 40 \si{cm^{3}} and 60 \si{cm^{3}} sizes is reported, showing stable pose prediction, except for some outliers if the size becomes to large.}
%			\label{fig:bb}
%		\end{center}
%	\end{figure*}
%	To evaluate the effect of the bounding box size on the algorithm accuracy, four different types of bounding boxes are defined for patch extraction. The first two are determined by the bounding cube size of 40 \si{cm^{3}} (default setting) and 60 \si{cm^{3}}. The other two are tight bounding boxes, which were designed to investigate the possible results on the patches coming from common object detectors, e.g. R-CNNs \cite{girshick2014rich,girshick2015fast,ren2015faster}, YOLO \cite{redmon2016you} and SSD \cite{liu2016ssd}. The first tight bounding box type one extracts tight cubic bounding boxes resulting in non-distorted object shapes of the maximal possible size. The other one simply takes the tight bounding box of the object and transforms it to a constant patch size by distorting the object. Examples of resulting image patches for different bounding box sizes of the cat object can be seen in Fig. \ref{fig:bb_patches}.
%	%Following the method of \cite{zakharov2017} we assume an initial guess of the object's bounding box is given by a detector and for training we extract patches accordingly. We center the object and extract bounding boxes of fixed sizes to create image patches for our training set. We virtually set a cube around the object's center to obtain tight bounding boxes covering the whole object.
%	%In addition, to analyze our method's robustness to different bounding box sizes and thus changing detector accuracies, we include various cube sizes in our experiments. Examples for resulting image patches of different bounding box sizes of the cat object can be seen in Figure \ref{fig:bb}.
%	\begin{figure}[t]
%		\begin{center}
%			\begin{subfigure}[b]{.21\linewidth}
%				\centering
%				\includegraphics[width=\linewidth]{images/cat_tight_distorted.png}
%				\caption{distorted}
%			\end{subfigure}
%			\begin{subfigure}[b]{.21\linewidth}
%				\centering
%				\includegraphics[width=\linewidth]{images/cat_tight.png}
%				\caption{tight}
%			\end{subfigure}
%			\begin{subfigure}[b]{.21\linewidth}
%				\centering        
%				\includegraphics[width=\linewidth]{images/cat_02.png}
%				\caption{40 \si{cm^{3}}}
%			\end{subfigure}
%			\begin{subfigure}[b]{.21\linewidth}
%				\centering
%				\includegraphics[width=\linewidth]{images/cat_03.png}
%				\caption{60 \si{cm^{3}}}
%			\end{subfigure}
%			
%			\caption{Different bounding boxes for the cat object. Various bounding box sizes where used to explore the robustness of our method to different detectors.}
%			\label{fig:bb_patches}
%		\end{center}
%	\end{figure}
%
%	We train our model using datasets with different bounding box sizes and report our results in Fig. \ref{fig:bb}, showing that we obtain none to little accuracy drop when using tight bounding boxes or larger cube sizes around the object, which leads us to assume that our method can be robust to various initial detector estimates and makes it independent of the detector used in the pipeline. 
%	Despite the promising results, we experienced some outliers and accuracy drops whenever the background to object ratio becomes rather large, as can be seen for example from the duck object results we report in Fig. \ref{fig:bb}.
	
	\subsection{Sensitivity to regularization parameter $\lambda$}
	Since our loss function includes a regularization parameter $\lambda$ balancing the two components of regression and manifold learning, we conducted experiments on the sensitivity of this parameter using ten objects of the LineMOD dataset. By choosing different values for $\lambda$ and thus weighting either the $L_{d}$ loss or the pose loss $L_{pose}$ more, we found that the results improve for nearest neighbor pose retrieval, if the two terms are equally weighted, and decreases when focusing more on the regression loss. Regarding regression, we observed similar results: improvement when additionally focusing on the $L_{d}$ loss, enhancing the feature representation and decrease, if the model is only trained on regression. Nevertheless, it can be seen that regression has a much stronger influence on the nearest neighbor pose retrieval in terms of performance than the other way around. Thus, to obtain an optimal balance, we set $\lambda = 0.5$ in our experiments.
	
	The results, depicted in Fig. \ref{fig:lambda}, emphasize our assumption that the two terms are beneficial to one another, i.e. both features and pose regression are mutually optimized. Note that we omit the regression result in case the model was only trained on the feature representation, since the regression layer in this case should not be included in training.
	
	
	
	


==> contents/method.tex <==
\section{Methodology}

%All text must be in a two-column format. The total allowable width of the
%text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
%cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
%$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
%first page) should begin 1.0 inch (2.54 cm) from the top edge of the
%page. The second and following pages should begin 1.0 inch (2.54 cm) from
%the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
%cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
%paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
%page.
\begin{figure*}[h]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{images/pipeline.png}
		\caption{Given an input depth image patch $\textbf{x}_i$, we create corresponding triplets ($\textbf{x}_i, \textbf{x}_j, \textbf{x}_k$) and pairs ($\textbf{x}_i, \textbf{x}_j$) to optimize our model on both manifold embedding, creating robust feature descriptors, and pose regression. Obtaining either a direct pose estimate $\textbf{q}$ or using the resulting feature descriptor for nearest neighbor search in the descriptor database.}
		\label{fig:pipeline}
	\end{center}
\end{figure*}
Our methodology, depicted in Fig. \ref{fig:pipeline}, starts with training a CNN model for a given training set $S_{train} = \{ \textbf{s}_1, \ldots, \textbf{s}_N \} = \{(\textbf{x}_1, {c}_1, \textbf{q}_1), \ldots, (\textbf{x}_N, {c}_N ,\textbf{q}_N)\}$ consisting of $N$ samples. Each sample $\textbf{s}$ comprises a depth image patch $\textbf{x} \in \mathbb{R^{\text{n} \times \text{n}}}$ of an object, identified by its class $c \in \mathbb{N}$, together with the corresponding pose vector, $\textbf{q} \in \mathbb{R^\text{4}}$, which gives the orientation represented by quaternions.
%\begin{equation}
%\textbf{q} = (x, y, z, w). 
%\end{equation}

Our objective is to model the mapping function $\phi: X \rightarrow Q$, thus for a given input $\textbf{x}$ the predicted pose vector $\hat{\textbf{q}}$ is obtained as 

\begin{equation}
	\hat{\textbf{q}} = \phi(\textbf{x}; \textbf{w}),
\end{equation}
where $\textbf{w}$ are the model parameters. While the primary objective is to obtain an accurate pose estimation for any unseen data, having a well clustered feature space is of high interest as well and can be used to identify the objects class, if needed. To achieve this, we model the problem as a multi-task learning, namely pose regression and descriptor learning. Thus the overall objective function can be written as

\begin{equation}
	L_{MTL} = (1 - \lambda) L_{pose} + \lambda L_{d},
\end{equation}
where $\lambda$ is a regularization parameter. $L_{pose}$ and $L_d$ are the objective functions for the pose regression task and the descriptor learning task respectively.
%-------------------------------------------------------------------------
\subsection{Regression}

During training, our CNN model maps a given input $\textbf{x}$ to a lower dimensional feature vector $f(\textbf{x}) \in \mathbb{R}^d$, i.e. the output of the last fully connected layer before it is further utilized to regress the pose using the following loss function:
\begin{equation}
L_{pose} = \|\textbf{q} - \frac{\hat{\textbf{q}}}{\| \hat{\textbf{q}} \|} \|_2^2,
\end{equation}
where $\| \cdot \|_2$ is the $l_2$-norm and $\textbf{q}$ is the corresponding ground truth pose.

%In particular we want to find the quaternion such that the pose loss is constrained by the triplet and pairwise term that were previously introduced:
%\begin{equation}
%\argmin_{\hat{q}} L_{pose}, \hspace{0.3cm}\text{s.t.}\hspace{0.2cm} \underbrace{L_{triplets} + L_{pairs}}_{L_{features}} \leq \epsilon.
%\end{equation}
%
%Reformulating this equation as an unconstrained optimization problem, we obtain
%\begin{equation}
%\argmin_{\hat{q}} L_{pose} +  \lambda L_{features},
%\end{equation}
%where $\lambda = 1$ if not otherwise stated.
%
%Overall we use the following function
%
%\begin{equation}
%L = L_{pose} + \lambda (L_{triplets} + L_{pairs}),
%\end{equation}
%giving our final loss function to train the neural network.

\subsection{Descriptor Learning}
%domain shift, compact clustering
%For comparison to the baseline method, the training set $S_{train}$ can be used to generate a %database of image feature descriptors for nearest neighbor search, which is then used to obtain %the best corresponding pose for an unknown test image. In order to efficiently regress the pose %robust feature descriptors $f(\textbf{x})$ have to be created.
To create robust feature descriptors, object identities as well as poses should be well distinguishable in the feature space, creating a compact clustering of object classes as well as a respective pose mapping within the clusters. As a second requirement, since we mainly train our model on synthetic images, we need to map synthetic and real images to the same domain to ensure generalization to real applications. Here, we use the triplet and pairwise loss, as introduced in \cite{wohlhart2015learning}. Overall, we obtain the following loss function $L_{d}$ for descriptor learning:
\begin{equation}
L_{d} = L_{triplets} + L_{pairs}.
\end{equation}
%Here we use the triplet loss function $L_{triplets}$ to train the neural network. 
As depicted in Fig. \ref{fig:pipeline}, our model is trained on a set of triplets $(\textbf{s}_i, \textbf{s}_j, \textbf{s}_k) \in T$, where sample $\textbf{s}_i$ (anchor) corresponds to the current depth image $\textbf{x}_i$  and $\textbf{s}_j$ (puller) is chosen so that the image corresponds to the same object $c_i$ viewed from a similar pose $\textbf{q}_j$. However, $\textbf{s}_k$ (pusher) is chosen so that the image $\textbf{x}_k$ corresponds either to a different object $c_k$ or the same object $c_i$, but viewed under a very different pose $\textbf{q}_k$. 
%Example images are visualized in Fig. \ref{fig:pipeline}. 
The resulting loss, $L_{triplets}$, defined over a batch of triplets is formulated as
\begin{equation}
	L_{triplets} = \mkern-18mu \sum_{(\textbf{s}_i,\textbf{s}_j,\textbf{s}_k) \in T} { \mkern-18mu max\left(0,1-\frac{||f(\textbf{x}_i)-f(\textbf{x}_k)||_2^2}{||f(\textbf{x}_i)-f(\textbf{x}_j)||_2^2+m}\right)},
\end{equation}
pulling viewpoints under similar poses close together and pushing dissimilar ones or different objects further away. As appeared in \cite{zakharov2017}, $m$ corresponds to a dynamic margin defined as:
\begin{equation}
	m = \begin{cases}
	2 \arccos (|\textbf{q}_i \cdot \textbf{q}_j|) &\text{if } c_i = c_j,\\
	\gamma &\text{else,}
	\end{cases}
\end{equation}
where  $\gamma > 2\pi$.
The dynamic margin ensures that objects of different classes get pushed farther away while the margin for the same objects depends on the angular distance between the current viewpoints $\textbf{q}_i$ and $\textbf{q}_j$.

In addition, the pair-wise loss $L_{pairs}$ is used to push together the sample feature descriptors of the same object under the same or very similar pose but with different backgrounds or coming from different domains (synthetic and real). The pair-wise loss is computed on pairs $(\textbf{s}_i, \textbf{s}_j) \in P$ and is defined as:
\begin{equation}
L_{pairs} = \sum_{(\textbf{s}_i,\textbf{s}_j) \in P} {||f(\textbf{x}_i)-f(\textbf{x}_j)||_2^2},
\end{equation}
$f(\textbf{x}_i)$ being the feature descriptor extracted from the neural network for image $\textbf{x}_i$.

%All printed material, including text, illustrations, and charts, must be
%kept within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches
%(22.54 cm) high.
%-------------------------------------------------------------------------


%\begin{table}
%	\begin{center}
%		\begin{tabular}{|l|c|}
%			\hline
%			Method & Frobnability \\
%			\hline\hline
%			Theirs & Frumpy \\
%			Yours & Frobbly \\
%			Ours & Makes one's heart Frob\\
%			\hline
%		\end{tabular}
%	\end{center}
%	\caption{Results.   Ours is better.}
%\end{table}


%When placing figures in \LaTeX, it's almost always best to use
%\verb+\includegraphics+, and to specify the  figure width as a multiple of
%the line width as in the example below
%{\small\begin{verbatim}
%	\usepackage[dvips]{graphicx} ...
%	\includegraphics[width=0.8\linewidth]
%	{myfile.eps}
%	\end{verbatim}
%}
%\pagebreak
